Terrorism & Democracy in Burkina-Faso

This article examines the political consequences of terrorism in Burkina Faso. Using a dataset combining geolocated terrorist events from ACLED (from 2015 to 2024) with public opinion data from Afrobarometer, I compare the effect of successful terrorist attacks on public support for democracy and authoritarian alternatives. The results reveal that successful terrorist attacks significantly increase support for military regimes, one man regimes, and one party systems, while decreasing support for democratic governance. These changes are most pronounced immediately after the attacks and persist over time. This suggests that terrorism has triggered a trade-off in public preferences between security and freedom. The study also reveals that terrorism erodes perceptions of key democratic values, particularly civil liberties and freedom of movement. Robustness tests confirm that weak institutions or a lack of political knowledge are not driving the results. The article highlights how terrorism in fragile democracies can undermine democratic resilience and accelerate authoritarian drift.

==> Graph_and_Tables/LatexTables/Table0.tex <==
\renewcommand{\tablename}{Table}

\begin{table}[htp]
    \centering
    \caption{List of the principal terrorist group in Burkina-Faso}

    \begin{tabular}{|c|c|}

    \hline
        Terrorist group &  Ideology \\
        \hline
        Al Mourabitoune Battalion & Salafi-Jihadism\\
        Ansaroul Islam & Salafi-Jihadism, Ethnic Insurgency\\
        Islamic State (Greater Sahara) & Salafi-Jihadism, Global Jihadism \\
Islamic State (Sahel) & Salafi-Jihadism, Regional Caliphate \\
Islamic State (West Africa) - Greater Sahara & Salafi-Jihadism, Anti-Western \\
JNIM: Group for Support of Islam and Muslims & Salafi-Jihadism, Pan-Sahelian Jihad \\
Katiba Macina & Salafi-Jihadism, Ethnic Grievance \\
\hline
    \end{tabular}
    \label{tab:tab1}
\end{table}


==> Graph_and_Tables/LatexTables/Table2d.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
            &\multicolumn{1}{c}{Military rule}&\multicolumn{1}{c}{Support democracy}\\
\hline
Treated $\times$ Event-time, -4&       -0.33         &        0.19         \\
            &      (0.39)         &      (0.37)         \\
[1em]
Treated $\times$ Event-time, -3&        0.36         &        0.36         \\
            &      (0.26)         &      (0.20)         \\
[1em]
Treated $\times$ Event-time, -2&       -0.45         &        0.19         \\
            &      (0.37)         &      (0.38)         \\
[1em]
Treated $\times$  Event-time, 0&       -0.17         &        0.14         \\
            &      (0.29)         &      (0.30)         \\
[1em]
Treated $\times$  Event-time, +1&        1.05\sym{***}&       -1.15\sym{***}\\
            &      (0.25)         &      (0.24)         \\
[1em]
Treated $\times$  Event-time, +2&        1.82\sym{**} &       -1.43\sym{**} \\
            &      (0.55)         &      (0.49)         \\
\hline
Treated $\times$ Post&0.90\sym{**}         &-0.81\sym{**}         \\
            &        0.29         &        0.28         \\
R-Squared   &        0.16         &        0.14         \\
N           &    11921.00         &    11775.00         \\
\hline\hline
\multicolumn{3}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{3}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}


==> Graph_and_Tables/LatexTables/Table2e.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
            &\multicolumn{1}{c}{Military rule}&\multicolumn{1}{c}{Support democracy}\\
\hline
Treated $\times$ Event-time, -5&        0.04         &        0.54\sym{***}\\
            &      (0.16)         &      (0.12)         \\
[1em]
Treated $\times$ Event-time, -4&       -0.23         &        0.15         \\
            &      (0.33)         &      (0.32)         \\
[1em]
Treated $\times$ Event-time, -3&        0.14         &        0.46\sym{***}\\
            &      (0.17)         &      (0.13)         \\
[1em]
Treated $\times$ Event-time, -2&       -0.39         &        0.13         \\
            &      (0.30)         &      (0.33)         \\
[1em]
Treated $\times$  Event-time, 0&       -0.26         &        0.10         \\
            &      (0.22)         &      (0.25)         \\
[1em]
Treated $\times$  Event-time, +1&        0.54         &       -0.53         \\
            &      (0.30)         &      (0.34)         \\
[1em]
Treated $\times$  Event-time, +2&        0.50         &        0.02         \\
            &      (0.51)         &      (0.53)         \\
\hline
Treated $\times$ Post&  0.26\sym{}         & -0.14\sym{}         \\
            &        0.22         &        0.22         \\
R-Squared   &        0.15         &        0.14         \\
N           &    12685.00         &    12512.00         \\
\hline\hline
\multicolumn{3}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{3}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}


==> Graph_and_Tables/LatexTables/Table2f.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
            &\multicolumn{1}{c}{Military rule}&\multicolumn{1}{c}{Support democracy}\\
\hline
Treated $\times$ Event-time, -3&        0.43         &        0.49\sym{*}  \\
            &      (0.27)         &      (0.24)         \\
[1em]
Treated $\times$ Event-time, -2&       -0.41         &        0.68         \\
            &      (0.37)         &      (0.40)         \\
[1em]
Treated $\times$  Event-time, 0&       -0.05         &        0.29         \\
            &      (0.31)         &      (0.32)         \\
[1em]
Treated $\times$  Event-time, +1&        0.24         &       -1.09\sym{***}\\
            &      (0.51)         &      (0.23)         \\
[1em]
Treated $\times$  Event-time, +2&        0.25         &       -1.17\sym{**} \\
            &      (1.01)         &      (0.44)         \\
[1em]
Treated $\times$  Event-time, +3&       -0.12         &       -0.30         \\
            &      (0.68)         &      (0.35)         \\
\hline
Treated $\times$ Post&  0.08\sym{}         &-0.57\sym{*}         \\
            &        0.54         &        0.25         \\
R-Squared   &        0.15         &        0.13         \\
N           &    11583.00         &    11484.00         \\
\hline\hline
\multicolumn{3}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{3}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}


==> Graph_and_Tables/LatexTables/Table2g.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
            &\multicolumn{1}{c}{Military rule}&\multicolumn{1}{c}{Support democracy}\\
\hline
Treated $\times$ Event-time, -4&        0.43         &        0.11         \\
            &      (0.31)         &      (0.25)         \\
[1em]
Treated $\times$ Event-time, -3&        0.56\sym{*}  &        0.35\sym{*}  \\
            &      (0.24)         &      (0.14)         \\
[1em]
Treated $\times$  Event-time, -2&        0.34         &        0.02         \\
            &      (0.32)         &      (0.26)         \\
[1em]
Treated $\times$  Event-time, 0&        0.16         &        0.07         \\
            &      (0.26)         &      (0.20)         \\
[1em]
Treated $\times$  Event-time, +1&        0.47\sym{*}  &       -0.74\sym{***}\\
            &      (0.21)         &      (0.14)         \\
[1em]
Treated $\times$  Event-time, +2&        0.50         &       -0.40         \\
            &      (0.31)         &      (0.26)         \\
[1em]
Treated $\times$  Event-time, +3&        0.34         &       -0.05         \\
            &      (0.25)         &      (0.15)         \\
\hline
Treated $\times$ Post& 0.37\sym{*}         &-0.28\sym{*}         \\
            &        0.15         &        0.12         \\
R-Squared   &        0.15         &        0.14         \\
N           &    10291.00         &    10198.00         \\
\hline\hline
\multicolumn{3}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{3}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}


==> Graph_and_Tables/LatexTables/Table2h.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
            &\multicolumn{1}{c}{Military rule}&\multicolumn{1}{c}{Support democracy}\\
\hline
Treated $\times$ Event-time, -3&        0.01         &        0.12         \\
            &      (0.09)         &      (0.21)         \\
[1em]
Treated $\times$ Event-time, -2&       -0.27         &       -0.15         \\
            &      (0.28)         &      (0.23)         \\
[1em]
Treated $\times$  Event-time, 0&       -0.36\sym{*}  &       -0.13         \\
            &      (0.16)         &      (0.18)         \\
[1em]
Treated $\times$  Event-time, +1&        0.17         &       -0.33         \\
            &      (0.20)         &      (0.20)         \\
[1em]
Treated $\times$  Event-time, +2&        0.02         &        0.13         \\
            &      (0.14)         &      (0.13)         \\
[1em]
Treated $\times$  Event-time, +3&       -0.18\sym{*}  &       -0.01         \\
            &      (0.07)         &      (0.08)         \\
\hline
Treated $\times$ Post& -0.09\sym{}         & -0.08\sym{}         \\
            &        0.08         &        0.10         \\
R-Squared   &        0.13         &        0.14         \\
N           &    15718.00         &    15593.00         \\
\hline\hline
\multicolumn{3}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{3}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}


==> Graph_and_Tables/LatexTables/Tableau2a.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
            &\multicolumn{1}{c}{Military rule}&\multicolumn{1}{c}{Support democracy}\\
\hline
Treated $\times$ Event-time, -3&        0.46         &        0.31         \\
            &      (0.24)         &      (0.21)         \\
[1em]
Treated $\times$ Event-time, -2&       -0.54         &        0.59         \\
            &      (0.36)         &      (0.37)         \\
[1em]
Treated $\times$  Event-time, 0&       -0.09         &        0.19         \\
            &      (0.26)         &      (0.32)         \\
[1em]
Treated $\times$  Event-time, +1&        1.10\sym{***}&       -1.25\sym{***}\\
            &      (0.24)         &      (0.24)         \\
[1em]
Treated $\times$  Event-time, +2&        2.00\sym{***}&       -1.65\sym{**} \\
            &      (0.55)         &      (0.53)         \\
\hline
Treated $\times$ Post&1.00\sym{***}         &-0.90\sym{**}         \\
            &        0.29         &        0.30         \\
R-Squared   &        0.15         &        0.14         \\
N           &    11098.00         &    10979.00         \\
\hline\hline
\multicolumn{3}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{3}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}

